Instance Shadow Detection

Instance shadow detection is a brand new problem, aiming to find shadow instances paired with object instances. To approach it, we first prepare a new dataset called SOBA, named after Shadow-OBject Association, with 3,623 pairs of shadow and object instances in 1,000 photos, each with individual labeled masks. Second, we design LISA, named after Light-guided Instance Shadow-object Association, an end-to-end framework to automatically predict the shadow and object instances, together with the shadow-object associations and light direction. Then, we pair up the predicted shadow and object instances, and match them with the predicted shadow-object associations to generate the final results. In our evaluations, we formulate a new metric named the shadow-object average precision to measure the performance of our results. Further, we conducted various experiments and demonstrate our method's applicability on light direction estimation and photo editing.

==> Figure_results.tex <==
\begin{figure*}[h]
	\centering
	%\vspace{-1.5mm}
	\includegraphics[width=0.99\linewidth]{figure/results_1.pdf}
	
	
	\begin{minipage}[t]{0.32 \linewidth}
		\centerline{\footnotesize (a) Relation Results}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (b) Ground Truth}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (c) Our Instance Shadow  Results}
	\end{minipage}
	
	\caption{}
	\label{fig:our_data}
	%\vspace{-3.5mm}
\end{figure*}

\begin{figure*}[]
	\centering
	%\vspace{-1.5mm}
	\includegraphics[width=0.99\linewidth]{figure/results_2.pdf}
		
	\begin{minipage}[t]{0.32 \linewidth}
		\centerline{\footnotesize (a) Relation Results}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (b) Ground Truth}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (c) Our Instance Shadow  Results}
	\end{minipage}
	
	\caption{}
	\label{fig:our_data}
	%\vspace{-3.5mm}
\end{figure*}


\begin{figure*}[]
	\centering
	\includegraphics[width=0.99\linewidth]{figure/results_3.pdf}
	
	\begin{minipage}[t]{0.32 \linewidth}
		\centerline{\footnotesize (a) Relation Results}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (b) Ground Truth}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (c) Our Instance Shadow  Results}
	\end{minipage}
	
	\caption{}
	\label{fig:our_data}
	%\vspace{-3.5mm}
\end{figure*}

\begin{figure*}[] 
	\centering
	\includegraphics[width=0.99\linewidth]{figure/results_4.pdf} 
	
	\begin{minipage}[t]{0.32 \linewidth}
		\centerline{\footnotesize (a) Relation Results}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (b) Ground Truth}
	\end{minipage}
	\begin{minipage}[t]{0.33 \linewidth}
		\centerline{\footnotesize (c) Our Instance Shadow  Results}
	\end{minipage}

	
	\caption{}
	\label{fig:our_data}
	%\vspace{-3.5mm}
\end{figure*}



==> tables_maskrcnn.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%							Tables_ 					       	%
%				    Created Time: 2019.10.21					%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{itemize}
%%  \item Baseline 1: Mask R-CNN trained by using shadow-object mask to output shadow-object association instances segmentation and box.
%  \item Baseline 1: Mask R-CNN trained by using shadow/object masks to output shadow/object instances segmentation and then use distance assumption to match shadow/object instances.
%  \item Baseline 2: 
%\end{itemize}





%%%%%%%%%%%%%%%%  Table 1 %%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[h]
%\centering
%\caption{Comparison with baseline 1 on relation box brach.}
%\label{tab: box}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{@{}ccccccc@{}}
%\toprule
%Method & AP & AP50 & AP75 & APs & APm & APl \\ \midrule
%Baseline 1 & 48.5 & \textbf{78.2} & 52.5 & \textbf{19.7} & \textbf{41.9} & 57.1 \\
%Baseline 2 & 38.7 & 56.8 & 42.1 & 11.0 & 29.0 & 49.6\\
%Our & \textbf{50.2} & 70.0 & \textbf{57.3} & 17.6 & 40.3 & \textbf{61.6} \\ \bottomrule
%\end{tabular}%
%}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%  Table 2 %%%%%%%%%%%%%%%%%%%%%%%

%\begin{table}[h]
%\centering
%\caption{Comparison with baseline 1 method on relation segm brach.}
%\label{tab: segm}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{@{}ccccccc@{}}
%\toprule
%Method & AP & AP50 & AP75 & APs & APm & APl \\ \midrule
%Baseline 1 & 38.5 & \textbf{68.9} & 37.8 & 6.1 & 29.5 & 47.5 \\
%Baseline 2 & 33.6 & 54.5 & 39.2 & 6.4 & 24.1 & 43.4 \\
%Our & \textbf{42.4} & 67.5 & \textbf{47.1} & \textbf{8.0} & \textbf{31.4} & \textbf{53.9} \\ \bottomrule
%\end{tabular}%
%}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%  Table 3 %%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[h]
%\centering
%\caption{Instance detection bounding box AP on test set.}
%\vspace{0.5mm}
%\label{tab: sobox}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{@{}ccccccc@{}}
%\toprule
%Method & AP & AP50 & AP75 & APs & APm & APl \\ \midrule
%Baseline 1 & \textbf{38.1} & \textbf{71.0} & 37.6 & 20.2 & 38.5 & \textbf{49.9} \\
%Baseline 2 & 37.0& 69.3 & 36.5 & 19.6 & 38.8 & 47.3 \\
%Our & \textbf{38.1} & 70.4 & \textbf{38.2} & \textbf{20.6} & \textbf{40.0} & 48.4 \\ \bottomrule
%\end{tabular}%
%}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%% Table 4 %%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[h] 
%\centering
%\caption{Instance detection mask AP on test set.}
%\vspace{0.5mm}
%\label{tab: somask}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{@{}ccccccc@{}}
%\toprule
%Method & AP & AP50 & AP75 & APs & APm & APl \\ \midrule
%Baseline 1 & 35.5 & 68.0 & 34.5 & 14.6 & 33.9 & 51.4 \\
%Baseline 2 & 36.4 & 67.4 & 35.5 & 15.5 & 35.9 & 52.1 \\
%Our & \textbf{37.0} & \textbf{68.5} & \textbf{36.7} & \textbf{16.6} & \textbf{36.9} & \textbf{53.3} \\ \bottomrule
%\end{tabular}%
%}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

